Efficient Topology-aware Data Augmentation for High-Degree Graph Neural Networks

In recent years, graph neural networks (GNNs) have emerged as a potent tool for learning on graph-structured data and won fruitful successes in varied fields. The majority of GNNs follow the message-passing paradigm, where representations of each node are learned by recursively aggregating features of its neighbors. However, this mechanism brings severe over-smoothing and efficiency issues over high-degree graphs (HDGs), wherein most nodes have dozens (or even hundreds) of neighbors, such as social networks, transaction graphs, power grids, etc. Additionally, such graphs usually encompass rich and complex structure semantics, which are hard to capture merely by feature aggregations in GNNs. Motivated by the above limitations, we propose TADA, an efficient and effective front-mounted data augmentation framework for GNNs on HDGs. Under the hood, TADA includes two key modules: (i) feature expansion with structure embeddings, and (ii) topology- and attribute-aware graph sparsification. The former obtains augmented node features and enhanced model capacity by encoding the graph structure into high-quality structure embeddings with our highly-efficient sketching method. Further, by exploiting task-relevant features extracted from graph structures and attributes, the second module enables the accurate identification and reduction of numerous redundant/noisy edges from the input graph, thereby alleviating over-smoothing and facilitating faster feature aggregations over HDGs. Empirically, TADA considerably improves the predictive performance of mainstream GNN models on 8 real homophilic/heterophilic HDGs in terms of node classification, while achieving efficient training and inference processes.

==> tex/pseudocode.tex <==
\section{Algorithmic Details}

==> tex/solution1.tex <==


\subsection{Connection Between GNNs and Network Embedding}

https://yangliang.github.io/pdf/www22.pdf

\subsection{Efficient Attribute Augmentation}

The augmented attribute matrix is $\widehat{\XM} = \XM \mathbin\Vert \AM \in \mathbb{R}^{n \times (d+n)}$, where $\mathbin\Vert$ denotes horizontal concatenation. After an MLP layer with weight matrix $\boldsymbol{\Theta}\in \mathbb{R}^{(d+n)\times h}$, we node features are
\begin{equation}
\HM^{(0)} = f_{\theta}(\widehat{\XM}) = \widehat{\XM} \boldsymbol{\Theta} \in \mathbb{R}^{n\times h}.
\end{equation}

Then feature propagation,
\begin{equation}\label{eq:H-K}
\HM^{(L)} = \sum_{\ell=0}^{L}{\alpha^\ell\NAM^\ell} \cdot \HM^{(0)} = \sum_{\ell=0}^{L}{\alpha^\ell\NAM^{\ell}} \cdot \widehat{\XM} \boldsymbol{\Theta}.
\end{equation}

\begin{lemma}
Let $\UM\boldsymbol{\Lambda}\UM^{\top}$ be the eigen-decomposition of $\NAM$. The following holds:
$\sum_{\ell=0}^{L}{\alpha^\ell\NAM^\ell} = \UM \left(\frac{1-(\alpha\boldsymbol{\Lambda})^{L+1}}{1-\alpha\boldsymbol{\Lambda}}\right) \UM^{\top}$.
\end{lemma}

Let $\widehat{\UM} = \UM\sqrt{\frac{1-(\alpha\boldsymbol{\Lambda})^{L+1}}{1-\alpha\boldsymbol{\Lambda}}}$. Eq. \eqref{eq:H-K} becomes
\begin{equation}
\HM^{(L)} = \widehat{\UM}\widehat{\UM}^{\top} \cdot \HM^{(0)} = \widehat{\UM}\widehat{\UM}^{\top} \cdot \widehat{\XM} \boldsymbol{\Theta} = \widehat{\UM}\cdot (\widehat{\UM}^{\top}\widehat{\XM})\cdot \boldsymbol{\Theta},
\end{equation}
where $\widehat{\UM}^{\top}\widehat{\XM}\in \mathbb{R}^{k \times (d+n)}$ if we perform $k$-largest eigen-decompsition.



\cite{sun2023feature}



